GarmentX: Autoregressive Parametric Representations for High-Fidelity 3D Garment Generation

This work presents GarmentX, a novel framework for generating diverse, high-fidelity, and wearable 3D garments from a single input image. Traditional garment reconstruction methods directly predict 2D pattern edges and their connectivity, an overly unconstrained approach that often leads to severe self-intersections and physically implausible garment structures. In contrast, GarmentX introduces a structured and editable parametric representation compatible with GarmentCode, ensuring that the decoded sewing patterns always form valid, simulation-ready 3D garments while allowing for intuitive modifications of garment shape and style. To achieve this, we employ a masked autoregressive model that sequentially predicts garment parameters, leveraging autoregressive modeling for structured generation while mitigating inconsistencies in direct pattern prediction. Additionally, we introduce GarmentX dataset, a large-scale dataset of 378,682 garment parameter-image pairs, constructed through an automatic data generation pipeline that synthesizes diverse and high-quality garment images conditioned on parametric garment representations. Through integrating our method with GarmentX dataset, we achieve state-of-the-art performance in geometric fidelity and input image alignment, significantly outperforming prior approaches. We will release GarmentX dataset upon publication.

==> Tex/Preliminaries.tex <==
\section{Preliminaries}
\subsection{Sewing Pattern Representation}
Each sewing pattern for a garment contains two parts of information: panel information and stitch information. Assuming each pattern consists of ${N_p}$ panels and each panel consists of ${N_e}$ edges, each edge includes several parameters that represent the starting point coordinates $({v_x},{v_y})$ of the edge and parameters related to the type of edge. Since each panel is closed, there is no need to store the endpoint coordinates. The parameters vary depending on the type of line: a straight line has no additional parameters, a quadratic Bézier curve has $2$ parameters representing the coordinates $({c_x},{c_y})$ of the Bézier control points, an arc has $3$ parameters $(r,l,d)$ representing the arc radius, whether it uses an arc greater than $180$ degrees, and the direction of the arc, and a cubic Bézier curve has $4$ parameters representing the coordinates $({c_{1x}},{c_{1y}},{c_{2x}},{c_{2y}})$ of the Bézier control points. Stitch information is defined as a set of one-to-one connections between the edge of one panel and the edge of another panel within the same garment.
\subsection{Sewing Pattern Generator}
In the real garment-making process, a clothing template is typically used. By adjusting the parameters of this template, such as the neckline shape (V-neck, Circle-neck, or others), the length of the pants, and the tightness of the cuffs, various types of garments can be created. Mimicking this process, each sewing pattern is generated by a sewing pattern generator \cite{korosteleva2021generating,korosteleva2023garmentcode} based on a template and a set of predefined parameters. The template defines the stitch information, while the parameters determine the type and shape of the garment, which in turn affects the panel information.
